Neural Abstraction-Based Controller Synthesis and Deployment

Abstraction-based techniques are an attractive approach for synthesizing correct-by-construction controllers to satisfy high-level temporal requirements. A main bottleneck for successful application of these techniques is the memory requirement, both during controller synthesis and in controller deployment. We propose memory-efficient methods for mitigating the high memory demands of the abstraction-based techniques using neural network representations. To perform synthesis for reach-avoid specifications, we propose an on-the-fly algorithm that relies on compressed neural network representations of the forward and backward dynamics of the system. In contrast to usual applications of neural representations, our technique maintains soundness of the end-to-end process. To ensure this, we correct the output of the trained neural network such that the corrected output representations are sound with respect to the finite abstraction. For deployment, we provide a novel training algorithm to find a neural network representation of the synthesized controller and experimentally show that the controller can be correctly represented as a combination of a neural network and a look-up table that requires a substantially smaller memory. We demonstrate experimentally that our approach significantly reduces the memory requirements of abstraction-based methods. For the selected benchmarks, our approach reduces the memory requirements respectively for the synthesis and deployment by a factor of $1.31\times 10^5$ and $7.13\times 10^3$ on average, and up to $7.54\times 10^5$ and $3.18\times 10^4$. Although this reduction is at the cost of increased off-line computations to train the neural networks, all the steps of our approach are parallelizable and can be implemented on machines with higher number of processing units to reduce the required computational time.

==> catalog.tex <==
% !TEX root = main.tex

\section{Description of Case Studies}
\label{app:catalog}
Description of the case studies used in this paper can be found in Tab.~\ref{tab:case_studies}.

\begin{table*}
	\tiny
	\centering
	%\caption{Catalog of case-studies considered in this paper.
	\caption{Catalog of models used to generate the finite abstractions in Sec.~\ref{sec:experiments}.
		\textmd{}
		\label{tab:case_studies}
	}
	
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{0.2em} % for the horizontal padding
	%\resizebox{1\columnwidth}{!}{
	\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
		\toprule
		\multirow{2}{*}{Case study}&\multirow{2}{*}{Dynamics of the model}& \multicolumn{4}{c}{Configuration (1)}&\multicolumn{4}{|c}{Configuration (2)}\\\cmidrule(l){3-10}
			&&$X$&$U$&$\eta_x$&$\eta_u$&$X$&$U$&$\eta_x$&$\eta_u$\\
		\midrule
		
		\multirow{1}{*}{2D car}& \multirow{2}{*}{$\begin{bmatrix}\dot\xb(1)\\\dot\xb(2)\end{bmatrix}\in\begin{bmatrix}\ub(1)\\\ub(2)\end{bmatrix}+W$}&$[0,5]^2$&$[-1,1]^2$&\multirow{2}{*}{$\begin{bmatrix}0.05\\0.05\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.23\\0.23\end{bmatrix}$}&$[0,10]^2$&$[-2,2]^2$&\multirow{2}{*}{$\begin{bmatrix}0.025\\0.025\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.23\\0.23\end{bmatrix}$}\\{$(\xb(1),\xb(2))$- position}&&&&&&&&&\\{$(\ub(1),\ub(2))$- speed}&$\tau=0.4$, $W=[-0.025,0.025]^2$&&&&&&&&\\
		
		\midrule
		
		\multirow{1}{*}{3D car}& \multirow{3}{*}{$\begin{bmatrix}\dot\xb(1)\\\dot\xb(2)\\\dot \xb(3)\end{bmatrix}\in\begin{bmatrix}\ub(1)\cos(\xb(3))\\\ub(1)\sin(\xb(3))\\\ub(2)\end{bmatrix}+W$}&$[0,5]^2\times$&$[-1,1]^2$&\multirow{3}{*}{$\begin{bmatrix}0.2\\0.2\\0.2\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.3\\0.3\end{bmatrix}$}&$[0,10]^2\times$&$[-1.5,1.5]\times$&\multirow{3}{*}{$\begin{bmatrix}0.1\\0.1\\0.1\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.2\\0.2\end{bmatrix}$}\\{$(\xb(1),\xb(2))$- position}&&$[-1.6, 1.6]$&&&&$[-\pi, \pi]$&$[-1, 1]$&&\\
		$\xb(3)$- angle&&&&&&&&&\\
		$\ub(1)$- speed&&&&&&&&&\\
		$\ub(2)$- turn rate&$\tau=0.3$, $W=\set{\textbf 0}$&&&&&&&&\\
		
		\midrule
		
		\multirow{1}{*}{4D car}& \multirow{4}{*}{$\begin{bmatrix}\dot\xb(1)\\\dot\xb(2)\\\dot \xb(3)\\\dot \xb(4)\end{bmatrix}\in\begin{bmatrix}\xb(4)\cos(\xb(3))\\\xb(4)\sin(\xb(3))\\\ub(1)\\\ub(2)\end{bmatrix}+W$}&{$[0,5]^2\times$}&$[-1,1]^2$&\multirow{4}{*}{$\begin{bmatrix}0.2\\0.2\\0.2\\0.2\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.3\\0.3\end{bmatrix}$}&{$[0,10]^2\times$}&$[-2,2]^2$&\multirow{4}{*}{$\begin{bmatrix}0.05\\0.05\\0.1\\0.1\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.2\\0.2\end{bmatrix}$}\\{$(\xb(1),\xb(2))$- position}&&$[-1.6,1.6]\times$&&&&$[-\pi,\pi]\times$&&&\\
		$\xb(3)$- angle&&$[-1,1]$&&&&$[-1,1]$&&&\\
		$\xb(4)$- speed&&&&&&&&&\\
		$\ub(1)$- turn rate&&&&&&&&&\\
		$\ub(2)$- acceleration control&$\tau=0.5$, $W=\set{\textbf 0}$&&&&&&&&\\
		
		\midrule
		
		\multirow{1}{*}{5D car}& \multirow{4}{*}{$\begin{bmatrix}\dot\xb(1)\\\dot\xb(2)\\\dot \xb(3)\\\dot \xb(4)\\\dot\xb(5)\end{bmatrix}\in\begin{bmatrix}\xb(4)\cos(\xb(3))\\\xb(4)\sin(\xb(3))\\\xb(5)\\\ub(1)\\\ub(2)\end{bmatrix}+W$}&{$[0,5]^2\times$}&$[-1,1]^2$&\multirow{4}{*}{$\begin{bmatrix}0.2\\0.2\\0.2\\0.2\\0.2\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.3\\0.3\end{bmatrix}$}&{$[0,10]^2\times$}&$[-2,2]^2$&\multirow{4}{*}{$\begin{bmatrix}0.05\\0.05\\0.1\\0.1\\0.1\end{bmatrix}$}&\multirow{2}{*}{$\begin{bmatrix}0.2\\0.2\end{bmatrix}$}\\{$(\xb(1),\xb(2))$- position}&&$[-1.6,1.6]\times$&&&&$[-\pi,\pi]\times$&&&\\
		$\xb(3)$- angle&&$[-1,1]\times $&&&&$[-1,1]\times$&&&\\
		$\xb(4)$- speed speed&&$[-1,1]$&&&&$[-1,1]$&&&\\
		$\xb(4)$- turn rate&&&&&&&&&\\
		$\ub(1)$- acceleration &&&&&&&&&\\
		$\ub(2)$- angular acceleration &$\tau=0.5$, $W=\set{\textbf 0}$&&&&&&&&\\
		\bottomrule
	\end{tabular}%}
\end{table*}

==> responses.tex <==
% !TEX root = main.tex

\section*{Revision Letter}
We would like to deeply thank the reviewers for reviewing our paper and providing us with the constructive comments and suggestions. We present below a detailed discussion of all the changes, comments, questions, and concerns raised by reviewers. The major modifications are highlighted in \textcolor{blue}{blue} color in the revised manuscript. %We also use red and blue colour in the response letter for referring respectively to the previous and current versions of the manuscript.
%Our responses to your specific questions are summarized as follows.
\subsection*{Changes}
We have carefully addressed all the comments in the revised manuscript. In particular,
\begin{itemize}
\item we have considered two additional case studies---whose dynamics are different from the multi-dimensional vehicles considered before---and showed that our method can significantly improve the memory requirements also on these case studies for both of the synthesis and deployment processes;
\item we have extended the related work section of our paper and included recent papers on neural-based controller synthesis, verification, and deployment;
\item we have extended the discussion section of the paper by including further points on different aspects of our method;
\item in the experimental section, we have demonstrated how different parameterizations can affect the performance of our method;  
\item we have modified and polished \Cref{fig:NN_vs_f,fig:ex_disconnected,fig:deployment} in order to address the reviewers concerns. Further, we have addressed all the other minor points raised by the reviewers.
\end{itemize}

\subsection*{Responses to the Questions}
\textbf{Generality of the provided case studies (Reviewers 1, 2, 3, 4)}. In order to demonstrate the effectiveness of our approach for dynamics other than the previously included multi-dimensional cars, we have reported results for two additional case studies (inverted pendulum and TORA). Both systems have been considered in different publications including the AINNCS category of the ARCH competition. Numerical results prove that our method has a very good performance also for these new case studies as reported quantitatively in the paper. 

\smallskip
\noindent
\textbf{Extending the related work (Reviewers 1, 2, 4)}. 
We have significantly extended the related work section of our paper. In brief, we have argued that
%
\begin{itemize}
\item the specifications studied in our paper are infinite horizon, while the ones considered in control systems with verified neural networks are finite horizon; 
our approach is based on computing an under-approximation of $\Pre$ and over-approximation of $\Post$ operators, thus applicable to any synthesis problem whose solution is characterized based on these operators;
\item our compression scheme provides strong correctness guarantees which would not be achievable by the existing methods such as reinforcement learning that use neural networks in order to scale the synthesis or deployment processes;
\item as opposed to the existing on-the-fly synthesis methods, our method is designed to be applicable to systems for which the analytical model is not available;
\item finally, our method can be applied on top of the existing symbolic BDD-based compression synthesis and deployment methods with appropriate adjustments.
\end{itemize}

\noindent
\textbf{Comparison with a baseline method (reviewer 4).}
We have demonstrated the effectiveness of our method on a number of case studies in compressing finite transition systems and controllers which are stored in the form of look-up tables. In the introduction and related work sections of our paper, we have discussed why other methods cannot be used to solve our problem. In below, we have listed our main arguments.
\begin{itemize}
\item While transition systems and controllers can be encoded using BDDs instead of look-up tables, the memory blow-up problem still exists for systems of higher dimensions. However, using our technique, we empirically show that the size of the computed representations is not necessarily affected by size of the original mapping. See for example Fig.~\ref{fig:results} (Left), wherein the memory required by the trained compressed representation stays at 488 kB, despite the fact that the required memory by the original transition system has increased by a factor of 5000.
\item Also, our synthesis setting is different from the one considered in references \cite{Reissig:2022,Girard:2022,Rungger:2022}, wherein memory-efficient synthesis methods are proposed based on a (compact) analytical description of the nominal dynamics of the system and its growth bound. We consider the case wherein the input is a huge finite transition system which can also be learned from simulations. 
\item Finally, while the control determinization and compression schemes proposed in \cite{Girard:2022, ZAPREEV:2018} are based on the BDD and ADD encodings of the controller, the only methodologically that is in a similar spirit as our deployment approach is the symbolic regression of \cite{ZAPREEV:2018}. As mentioned by the authors of \cite{ZAPREEV:2018}, their regression-based method is not able to represent the original controller with an acceptable accuracy. Our superior performance is mainly because of our classification-based formulation, as opposed to a regression-based formulation.
%\textcolor{red}{This is not a good line of reasoning. You have space. Why not clarifying it now in this version? Eliminate the sentence.}
%\textcolor{red}{Why didn't we make a quantitative comparison with \cite{ZAPREEV:2018}. We need to modify the last part.}
\end{itemize}

\smallskip
\noindent\textbf{Parametrization of the neural networks (Reviewers 1, 4).} We have added a discussion on the selection of thehyperparameters in our approach. We have also added a new figure (Fig.~\ref{fig:parametrization}) that shows the effect of changing the depth of the neural network on the error. In summary, increasing the complexity of the neural network by increasing the number of neurons per layer or depth leads to a better performance.
%
The neural networks employed in our setting are not supposed to make any generalization over unseen data. Therefore, our approach does not suffer from over-parametrization of the neural networks.
%This is demonstrated in Fig.~\ref{fig:parametrization} by providing the error as a function of the depth of the neural representation for the 3D car example.

\smallskip
\noindent\textbf{Backpropagation through the max operation (Reviewer 4).} We first note that the $max$ operator is not part of the trained neural network.
We define the MSE error based on the mismatch error between the output vector of the neural network, which is a real-valued vector, and the reference vector, which is the vector with ones at the entries associated to the valid control inputs and zeros elsewhere.
%We define the MSE error based on the mismatch error between the reference vector---the vector with ones at the entries associated to the valid control inputs and zeros elsewhere--- and the output vector of the neural network---that is a real valued vector.
The considered error is of type $\ell_2$ norm with respect to the proposed (continuous) normed space. Defining $\ell_2$ or $\ell_1$ norm in the original setting will not work as the original output space---that is the space of valid control input sets---is discrete. The $max$ operator is applied to the output of the neural network and is not considered throughout the training phase.

\smallskip
\noindent\textbf{Possibility for application of invertible neural networks (Reviewer 4).} The idea of using invertible neural networks instead of training two separate neural networks is certainly interesting. However, given the specific application and inherent differences between our approach and the successful experiences with invertible neural networks, it is currently not obvious to us that the same performance would be accessible. We have added this point to the discussion section of our paper as a potential future research direction.

\smallskip
\noindent\textbf{Soundness of the corrected neural controller (Reviewer 4).} 
Our deployment method preserves soundness.
The input to our deployment approach is a formally guaranteed controller computed by any abstraction-based method. We train a neural representation that maps the states to a control input. This control input is valid for majority of the states. For the states that the control input is not valid, we keep the set of valid control inputs from the original controller and store them as a small look-up table. Therefore, the final corrected neural controller in Eq.~\eqref{eq:C_hat_def} is sound with respect to the original controller.

